Locally Differentially Private Heavy Hitter Identification

The notion of Local Differential Privacy (LDP) enables users to answer sensitive questions while preserving their privacy. The basic LDP frequent oracle protocol enables the aggregator to estimate the frequency of any value. But when the domain of input values is large, finding the most frequent values, also known as the heavy hitters, by estimating the frequencies of all possible values, is computationally infeasible. In this paper, we propose an LDP protocol for identifying heavy hitters. In our proposed protocol, which we call Prefix Extending Method (PEM), users are divided into groups, with each group reporting a prefix of her value. We analyze how to choose optimal parameters for the protocol and identify two design principles for designing LDP protocols with high utility. Experiments on both synthetic and real-world datasets demonstrate the advantage of our proposed protocol.

==> ack.tex <==
\section{Acknowledgment}
This paper is based upon work supported by the United States National Science Foundation under Grant No. 1640374

==> comp_thres.tex <==


\section{Protocol Analysis and Optimization}
\label{sec:analyze}

We analyze and compare different protocols in this section. 
Both \product and \itergroup satisfy local differential privacy, and the complexity of them are already clear in the description. In this section, we focus on utility of the protocols. All the analysis are supported by empirical results.

Given $\delta$, we first study the probability a candidate with frequency $f$ is identified as a heavy hitter. Then we calculate the expected number of heavy hitters (true positive) and non-heavy hitters (false positive) a protocol will give. In the end, we try to optimize parameters for the protocols.


We focus on \itergroup in this section, and the analysis of \product can be easily derived.

%\subsection{Privacy}
%Although all protocols satisfy local differential privacy. There are some slight differences between them.
%
%No partial result is leaked to any user in protocols that use hash functions (i.e., \simhash). On the other hand, for \product and \itergroup, the heavy hitters in some segments are sent to some users, which leaks some intermediate results. However, this can be avoided by using hash functions: instead of sending partial candidates to users, the aggregator first applies a hash function to the heavy hitters (with a big range so that collision happens with little probability), and then sends the hashed value; the users will indicate which hashed value his original answer is (with perturbation). Therefore, heavy hitters in many segments is protected, and heavy hitters in few segments does not matter too much.



%\subsection{Efficiency}
%
%For computation, \simhash is slow in that multiple channels are used for collision resistance, and \itergroup is slower than \product in that different segments cannot be parallelized.

%\subsection{Utility}


\begin{comment}
	

\subsubsection{\simhash}
Suppose the length of a value is $m$, and the segment size is $s$. For simplicity, assume the probability of collision is zero for now. We first needs to look at how large is $p(s)$, the probability a heavy hitter with frequency $f$ is identified in one segment.

The value length is $m$, and segment length is $s$, so there should be $g=m/s$ segments altogether.
Therefore, for each segment, there are $n'=n/g$ users reporting. Among them, approximately $n'f$ users have the heavy hitter (\says{tianhao}{we assume the $nf$ users are partitioned into each group equally likely, which is not true, but this assumption should not affect too much.}), and all the other $n'(1-f)$ users randomly select one value to report. We can regard this as a summation of $n'(1-f)$ binomials with parameter $\frac{1}{2^s}$. 

The aggregation process remains the same, but after we get the result, we may want to subtract $\frac{n'}{2^s}$ from each of them. \says{tianhao}{and thus we may need to rescale, so that the mean does not change etc. However, the mean of non-heavy hitters is different.}

We use Normal distribution to approximate this summation of Binomials, which has mean 
Suppose we use a threshold 
\[
T=\Phi^{-1}\left(1-\frac{1}{20\cdot 2^s}\right) \sqrt{\sigma^2\cdot n'},
\] 
which is used in \rappor~\cite{rappor,rappor2}, and $\sigma$ is the variance of a single item. We want to know what is the probability the estimated frequency $n'f'$ of a heavy hitter is less than $T$? Note that now $n'f'$ is a Normal distribution with mean $n'f$ and variance $\sigma^2 n'$.

\begin{align*}
p(s)&=\Pr{n'f'\geq T}\\
&=1-\Phi\left(\frac{\Phi^{-1}\left(1-\frac{1}{20\cdot 2^s}\right) \sqrt{\sigma^2\cdot n'}-n'f}{\sigma\sqrt{n'}}\right)\\
&=1-\Phi\left(\Phi^{-1}\left(1-\frac{1}{20\cdot 2^s}\right) -\sqrt{ns/m}f/\sigma\right)
\end{align*}

$\sigma$ is fixed given an LDP primitive, thus the probability a heavy hitter is identified: $p^{\frac{m}{s}}(s)$ is a function of $s$.


Assumptions so far:
\begin{enumerate}
	\item Different segments are considered independently, while in reality they may be related.
	\item Some approximation in variance analysis: we assume $n'(1-f)/2^s$ users take the value the same as the heavy hitter.
	\item Use Normal distribution to approximate summation of Binomials.
	\item Use a threshold to analyze the probability, where we use the one with highest in experiment.
\end{enumerate}
\end{comment}


\subsection{Identification Probability}
\label{subsec:iden_prob}


%Fixing the number of users $n$, domain size $2^m$, privacy budget $\epsilon$, and a fixed threshold constant $T$, the probability the heavy hitter is identified is a function of segment length $s$. 
%The protocol that uses a larger segment size $s$ will have a better chance of identifying a heavy hitter with the same frequency $f$.

%Protocols \product, \itergroup, and \simhash are included in this analysis. We will discuss the effect of error correction code (which was proposed by the original \hash method) later in this section. Protocol \rappor is slightly different but it uses far more groups (${{m/s}\choose{2}}$ instead of $2m/s-1$ in \product and \itergroup) and thus is expectedly less efficient. We will discuss it later.

Recall that \itergroup works phase by phase, with each phase outputs the frequent patterns in a larger segment. 
A value is identified as a heavy hitter if every part of it is identified in each corresponding phase.
%Users are partitioned into groups; each group participates in a phase.
Assume there are $n_1$ users participating in the first phase, now we analyze a value's identification probability in the first phase.
Consider a value $v_i$ with frequency $f_i$. Recall that we will pick values whose estimated count is above a threshold. For $v_i$, we need
$
\tilde{c}(v_i)>\delta\cdot n_1.
$
In the frequency estimator we use, the estimated value is the rescaling of the ``support'' it receives, thus, we have:
\begin{align*}
&\tilde{c}(i)= \frac{I_{v_i} - qn_1  }{p - q}>\delta n_1\\
\implies &I_{v_i} > qn_1+(p-q)\delta n_1.
\end{align*}
Suppose $n_f$ is the number of users with value $v_1$ in this group. $I_{v_i}$ will be composed of two parts: $I_1$ is received from the $n_f$ users. They each supports with probability $p$. $I_2$ comes from the other $n_1-n_f$ users that will each contribute with probability $q$. Therefore, \Pall{i}{1}, the probability value $v_i$ is identified in the first phase, equals the probability $I_1+I_2>\delta n_1$. We use $f(x;n,p)$ to denote the probability mass function of the binomial distribution. Therefore, we have:
\begin{align*}
\Pall{i}{1}=&\sum_{I_1=0}^{n_f}f\left(I_1;n_f,p\right)
\sum_{I_2=\delta n_1-I_1}^{n_1-n_f}f\left(I_2;n_1-n_f,q\right)
\end{align*}

Note that we assign users randomly into each group. Therefore, $n_f$ is summation of $n_s$ binomial variable with probability $f_i$. Thus,
\begin{align*}
\Pall{i}{1}=&\sum_{n_f=0}^{n_1}f(n_f;n_1,f_i)
\sum_{I_1=0}^{n_f}f\left(I_1;n_f,p\right)
\sum_{I_2=\delta n_1-I_1}^{n_1-n_f}f\left(I_2;N-n_f,q\right)
\end{align*}

In fact, $I_{v_i}$ can be viewed as the summation of one kind of binomials: 
The $n_1$ users will take value $v_i$ with probability $f_i$. Conditioned on that, they will support $I_{v_i}$ with probability $p$. 
If we use $F(x;n,p)$ to denote the cumulative density function of $n$ bernoullis with probability $p$.
\Pall{i}{1} equals to the cumulative density function where $I_{v_i}>\delta n_1$.
Moreover, we can approximate this using normal distribution with mean $\mu_1[i]=n_1(fp+(1-f)q)$ and variance $\sigma_1[i]=\sqrt{n_1(fp+(1-f)q)(1-fp-(1-f)q)}$.
Thus, we can simplify \Pall{i}{1} as:
\begin{align}
\Pall{i}{1}=&1-F((p-q)\delta n_1+n_sq;n_1,f_ip+(1-f_i)q)\nonumber\\
\sim &1-\Phi\left(\frac{T(p-q)+n_sq-\mu_1[i]}{\sigma_1[i]}\right)\label{eq:normal}
\end{align}
where $\Phi(x)$ is the cumulative density function of standard normal distribution. 


%The probability that a heavy hitter with probability $f$ is identified, varying number of total users, privacy budget and value length is given in Table~\ref{table:com_ana} (only compares segment length $1$ vs $8$, $Q=0.5$). 
%Note that the results match with the those given in Table~\ref{table:com}.
%
%In Figure~\ref{fig:comp_1000000} and \ref{fig:comp_10000000}, the identification probabilities are shown varying epsilon and the original probability, respectively.

\begin{comment}
\subsection{Significance Threshold}
\label{subsec:significance}
Due to the fact of the added noise, it is possible that an infrequent domain is overwhelmed by noise. A significance test is supposed to eliminate those possibly resulted from noise.
Suppose we want the expected false positives is smaller than $\alpha$. By Equation~\ref{eq:normal}, we will have 
\[
\EV{FP}\sim 2^s\left(1-\Phi\left(\frac{T-n_sq}{\sqrt{n_sq(1-q)}}\right)\right)\leq \alpha
\] 
the expected false positives assuming approximately $2^s$ values, each having zero probability. Simplifying this equation gives us
\[
T\geq n_sq+\Phi^{-1}\left(1-\frac{\alpha}{2^s}\right)\sqrt{n_sq(1-q)}
\]

%\subsection{An Upper Bound}

%We exam the probability a value $v$ with probability $f$ is identified in a group of size $n_s$.
%We first rewrite Equation~\ref{eq:single}. 
%Since we assign users randomly into each group, and the value appears with frequency $f$, any user's value will be $v$ with probability $f$. 
%If the user has the heavy hitter, he will report faithfully with probability $p$, and if he does not hold the value, the probability he report the heavy hitter (he lies, but it's coincidently the heavy hitter we are considering) is $q$. Note that $p$ and $q$ depends on the LDP primitive we are using.




%In this section, we first measure the expected false positives fixing the threshold. The threshold is set so that the top $k$ most frequent values can be identified with probabilities greater than $90\%$. Fixing $T$, we measure the probability every other value is identified in \textbf{one} group, and take their sum as the expected false positives.

If we require the expected overall false positives are below $\gamma$, we will have 
\begin{align*}
\EV{FP}\sim & 2^s\left(1-\Phi\left(\frac{T-n_sq}{\sqrt{n_sq(1-q)}}\right)\right)^g\leq \gamma\\
\implies T\geq & n_sq+\Phi^{-1}\left(1-\left(\frac{\gamma}{2^s}\right)^{1/g}\right)\sqrt{n_sq(1-q)}
\end{align*}

We assume a zipf's distribution $\Pr{v=h_i}=\frac{(i+20)^{-1.5}}{\sum_{j=0}^{\infty}(j+20)^{-1.5}}$. 

Note that the distribution of any dataset is discrete, therefore, the optimal threshold should depend on the distribution of the underlying dataset. For example, when we use the zipf's distribution, the parameter affects the shape of the distribution. \todo{show and explain the shape.} Note that one approximation we use is that we assume a uniform distribution among the less frequent values that are not under test. That is, when $s=8$, there are at most $256$ values, and the probabilities of them must sum up to one. The summation of densities of values that are ranked $257$ to $\infty$ are divided equally into all the $256$ values under test. This may result inaccuracies of the analysis.

%When all possible values in a segment is too few, summation of zipf's distribution does not sum up to one. There must be some collision within the segment. For the $k$ top hitters, we are conservative in that we assume there are no collision. For the rest of the values, we divide the remaining probability uniformly to each value. This will result an upper bound of the expected false positives.
\end{comment}


\subsection{Optimization}
Given a threshold, we want to compare different methods according to their accuracies, measured by the expected \fone score. For each method, there is an optimal configuration that achieves the best accuracy. In this section, we try to find the optimal configuration for \itergroup. 
%The analyses for other methods are similar.

Without loss of generality, we assume the frequent values of the dataset are randomly distributed; $f_i$ is the probability of the $i$-th most frequent value.
Given the threshold $\delta$, we assume $t$ is the number of real true positives in this dataset, that is, $\Pr{t}>\delta$, and $\Pr{t+1}>\delta$.
If we denote $v_i$ as the $i$-th most frequent value in the dataset, the ideal output is $V_{ideal}=\{v_1,v_2,\ldots,v_t\}$.

In practice, this ideal scenario is hard to achieve, because the true positives may not be identified, and some false positives may be incorrectly identified. 
Given the real output $V_{real}$, we calculate the \fone score:
$$\fone = 2\cdot\frac{1}{\frac{1}{\mbox{precision}}+\frac{1}{\mbox{recall}}},$$
where precision is defined as $\frac{|V_{real}\cap V_{ideal}|}{|V_{real}|}$, and recall is defined as $\frac{|V_{real}\cap V_{ideal}|}{|V_{ideal}|}$.
Thus 
$$\fone=\frac{2|V_{real}\cap V_{ideal}|}{|V_{ideal}|+|V_{real}|}.$$
If we define \etp $=\EV{|V_{real}\cap V_{ideal}|}$ as the expected number of true positives, and \efp $=\EV{|V_{real}\setminus V_{ideal}|}$ as the expected number of false positives, by the linearity of expectations, $$\EV{\fone}=\frac{2\etp}{t+\etp+\efp}.$$


\itergroup works phase by phase. In each phase, we use existing results to estimate a segment. The possible parameters for a phase $k$ can be the number of users assigned in this phase, $n_k$, the threshold, $\delta_k$, and the length of segment under estimation, $s_k$. Note that in protocol description, we assume $n_k=n/g$ for all phases, $\delta_k=\delta$ for all phases, and $s_k$ is increasing, e.g., $s_1=16$ and $s_{i+1}-s_{i}=8$ for $i\geq 1$.

%In phase $k$, we analyze segment of length $s_k$. 
When $s_k$ is small, i.e., $2^{s_k}$ is smaller than all possible values in the dataset, by the pigeon-hole principle, there exists more than one values that share the same pattern in the current segment. If we analyze value $v_i$, the original frequency of its pattern in the current segment is $f_i$. Since we assume the values are randomly distributed, the expected probability any other value also takes $v_i$'s pattern is $1/2^{s_k}$. Thus, the expected frequency of $v_i$'s pattern after considering collision is 
$$\Prs{i}{k}=f_i+(1-f_i)/2^{s_k}=1/2^{s_k}+f_i(2^{s_k}-1)/2^{s_k}.$$

Given the expected frequency, we can calculate the probability it is identified in one phase using Equation~\ref{eq:normal}, conditioned on the fact it is identified in previous phases. Since each phase is independent, the identification probability in phase $k$ is the product of identification probabilities in all phases up to $k$.


Therefore, the expected number of true positives in phase $r$ is summation of probabilities of all the $t$ values, where the probability is computed as the product of all $r$ phases:
\begin{align*}
\etp=&\sum_{i=1}^{t}\left(\prod_{k=1}^{r}\Pall{i}{k}\right),
\end{align*}
where $\mu_k[i]=\Prs{i}{k}n_k(p-q)+n_kq$, $\sigma_k[i]=\sqrt{n_k\Pri{i}{k}(1-\Pri{i}{k})}$, and $\Pri{i}{k}=\Prs{i}{k}(p-q)+q$.
\begin{comment}
\begin{align*}
\etp=&\sum_{i=1}^{t}\prod_{k=1}^{r}\left(1-\Phi\left(\frac{ \delta_kn_k(p-q)-n_kq-\Prs{i}n_k(p-q)+n_kq}{\sqrt{n_k\Pri{i}(1-\Pri{i})}}\right)\right)\\
=&\sum_{i=1}^{t}\prod_{k=1}^{r}\left(1-\Phi\left(\sqrt{\frac{n_k}{\Pri{i}(1-\Pri{i})}} (p-q)(\delta_k-\Prs{i})\right)\right)
\end{align*}
\end{comment}
 
%In \itergroup, each phase $k$ explore $s_k-s_{k-1}$ new segment.
Suppose there are $d_r$ values to be considered in phase $r$. We assume these are the most frequent $d_r$ values in the distribution. 
Now we try to calculate the number of candidates that can be identified. 
For the top few values, they are frequent, thus the probability each of them is identified throughout all the $r$ phases is still high.
For the other values, their frequencies are not high enough. Consequently, the probability any of them is identified is nearly zero. In fact, it is highly likely these values are just random infrequent values. Therefore, the probability it is identified in phase $r$ does not depend on the condition it is identified in previous phases.
As a result, when calculating the expected number of identified values, we compare the probability a frequent value is identified through all phases, and the probability a random infrequent value is identified in the current phase, and pick the larger of the two as the expected value.
Formally, the expected number of identified values are:
\begin{align*}
c_r=\sum_{i=1}^{d_r}\max\left(\prod_{k=1}^{r}\Pall{i}{k}, \Pall{0}{r}\right),
\end{align*}
where $\mu_r[0]$ and $\sigma_r[0]$ are used to denote the mean and standard deviation of a random infrequent value $\Prs{0}{r}\sim 1/2^{s_r}$.

Once these $c_r$ values are identified as candidates in phase $r$, the protocol moves on the phase $r+1$ where an additional $s_{r+1}-s_r$ bits are examined. The values to be tested are the , thus $d_{r+1}=c_r\cdot 2^{s_{r+1}-s_r}$.

Suppose there are $r$ phases in the protocol, in the end, $V_{real}$ of size $c_r$ will be returned by the protocol. The expected number of final false positives is thus $c_r-\etp$. Given all the parameters $n_k$ and $\delta_k$ for any phase $k$ equals $1$ up to $r$, we therefore can calculate the final \fone score. The overall optimization problem becomes to vary the $n_k$ and $\delta_k$ values in order to maximize the final \fone score:

%There are $2^s$ possible segment patterns. It is possible a collision, where two values have the same pattern for this segment, happens. 
%For simplicity, we assume $r \ll 2^s$, thus no true positive collision will happen. Therefore, the expected number of true positives is $\etp(\delta_k,n_k)=\sum_{i=1}^{r} \Phi\left(\frac{\delta_k n_k-n_k(f_ip+(1-f_i)q)}{\sqrt{n_k(f_ip+(1-f_i)q)(1-(f_ip+(1-f_i)q))}}\right)$, where $\delta_k$ is the threshold for the current phase, and $n_k$ is the number of users assigned in this phase. If we rewrite $f_ip+(1-f_i)q$ as $\Prs{i}$, we will have $\etp(\delta_k,n_k)=\sum_{i=1}^{r}\Phi\left(\frac{ \sqrt{n_k}(\delta_k-\Prs{i})}{\sqrt{\Prs{i}(1-\Prs{i})}}\right)$.
%A value is output if it is identified in all phases. Thus the expected number of final true positives is 
%
%The expected number of false positives is estimated similarly, but note that there are far less patterns to consider than all possible values, which means there is high probability of collisions to happen. Moreover, the probability changes: For the first few phases, we analyze a short segment, but for the next few phases, we analyze long segments, while testing similar amount of candidates, thus the probabilities of false positives to be tested will drop to nearly zero, making the collision probability drop.
%
%To summarize, the number of true positives will drop phase by phase, but the number of false positives will not drop after a certain phase. For simplicity, we assume the the false positives have zero probability in the
%
%The assumptions made so far:
%\begin{itemize}
%	\item \itergroup is used.
%	\item Users are partitioned equally to answer each question.
%	\item The same threshold $\delta$ is used in each phase.
%	\item The first 
%\end{itemize}

\begin{align*}
\mbox{input: }
& n\mbox{ is number of users}\\
&\epsilon\mbox{ as privacy budget and } p=\frac{1}{2}, q=\frac{1}{e^\epsilon+1}\\
&m\mbox{ is length of binary representation of input}\\
&\{f_1,f_2,\ldots,f_{2^m}\}\mbox{ is the dataset distribution s.t., } f_1>f_2>\ldots>f_{2^m} \mbox{ and } \sum_{i=1}^{2^m}f_i=1\\
&\delta\mbox{ is the threshold (the goal is to identify values above it)}\\
&t\mbox{ is the largest number s.t., }f_t>\delta\mbox{ ($t$ is also the ideal number of true positives)}\\
%&t=\underset{i\in [2^m]}{\argmax}\; f_i>\delta\\
\mbox{choose: }
& r \in\mathbb{Z^+}\mbox{ is the number of phases}\\
&\forall k\in\{1,2,\ldots,r\}, \\
&\;\;\;\;\;\;s_k\in\mathbb{Z}\mbox{ is segment length in phase } k\\
&\;\;\;\;\;\;n_k\in\mathbb{Z}\mbox{ is number of users assigned to phase } k\\
&\;\;\;\;\;\;\delta_k\in\mathbb{Q}\mbox{ is threshold used in phase } k\\
\mbox{subject to: }
&0<s_1<s_2<\ldots<s_r=m\\
&\sum_{k=1}^{r}n_k=n\\
\mbox{maximize: }& \EV{\fone}=\frac{2\etp}{t+\etp+\efp} \\
\mbox{where: }
&\etp=\sum_{i=1}^{t}\left(\prod_{k=1}^{r}\Pall{i}{k}\right)\\
&\efp=c_r-\etp\\
&\forall k\in\{1,2,\ldots,r\}, \forall i\in\{0,1,2\ldots,2^m\}(\mbox{define }c_0=1, s_0=0, f_0=0):\\
&\;\;\;\;\;\; c_k= \sum_{i=1}^{d_k}\max\left(\prod_{\ell=1}^{k}\Pall{i}{\ell}, \Pall{0}{k}\right)\\
&\;\;\;\;\;\;\Pall{i}{k}=1-\Phi\left(\frac{ n_k(\delta_k(p-q)-q)-\mu_k[i]}{\sigma_k[i]}\right)\\
&\;\;\;\;\;\;\mu_k[i]=\Prs{i}{k}n_k(p-q)+n_kq\\
&\;\;\;\;\;\;\sigma_k[i]=\sqrt{n_k\Pri{i}{k}(1-\Pri{i}{k})}\\
&\;\;\;\;\;\;\Pri{i}{k}=\Prs{i}{k}(p-q)+q\\
&\;\;\;\;\;\;\Prs{i}{k}=f_i+(1-f_i)/2^{s_k}\\
&\;\;\;\;\;\;d_{k}=c_{k-1}\cdot 2^{s_{k}-s_{k-1}}\\
%&\;\;\;\;\;\;c_0=1, s_0=0, f_0=0\\
\end{align*}

Except the last phase, each phase is similar in terms of input and output. We expect the difference in the initial phases does not influence the final results much, thus it is reasonable to assume the initial phases use the same parameter.
We simplify the above general optimization problem into the following simpler one:
\begin{align*}
\mbox{input: }
& n\mbox{ is number of users}\\
&\epsilon\mbox{ as privacy budget and } p=\frac{1}{2}, q=\frac{1}{e^\epsilon+1}\\
&m\mbox{ is length of binary representation of input}\\
&\{f_1,f_2,\ldots,f_{2^m}\}\mbox{ is the dataset distribution s.t., } f_1>f_2>\ldots>f_{2^m} \mbox{ and } \sum_{i=1}^{2^m}f_i=1\\
&\delta\mbox{ is the threshold (the goal is to identify values above it)}\\
&t\mbox{ is the largest number s.t., }f_t>\delta\mbox{ ($t$ is also the ideal number of true positives)}\\
\mbox{choose: }
& r \in\mathbb{Z^+}\mbox{ is the number of phases}\\
&\theta\in\mathbb{Q}\mbox{ is segment length in phase } k\\
&\theta_r\in\mathbb{Q}\mbox{ is segment length in phase } r\\
\mbox{subject to: }
&(C\cdot 2^{s}-t)e^{-\frac{\theta^2n^2}{Var\cdot r}}=C-t\mbox{ (Chaining Constraint)}\\
&\implies C=\frac{t\left(1-e^{-\frac{\theta^2n^2}{Var\cdot r}}\right)}{\left(1-e^{\frac{m\ln 2}{r}-\frac{\theta^2n^2}{Var\cdot r}}\right)}\\
&\implies e^{\frac{m\ln 2}{r}-\frac{\theta^2n^2}{Var\cdot r}}<1\\
&\implies \frac{m\ln 2}{r}-\frac{\theta^2n^2}{Var\cdot r}<0\\
&\implies \theta>\sqrt{\frac{m}{n}}\left(\frac{2\sqrt{\ln 2}e^{\epsilon/2}}{e^\epsilon-1}\right)\\
&\left(2^{s_1}-t\right)e^{-\frac{(f-\theta)^2n^2}{Var\cdot r}}=C-t\\
&P_f=\left(1-e^{-\frac{(f-\theta)^2n^2}{Var\cdot r}}\right)^{r-1}\left(1-e^{-\frac{(f-\theta_r)^2n^2}{Var\cdot r}}\right)\geq 0.9\mbox{ (True Positive Constraint)}\\
&FP_r=C\cdot 2^{s_r}\cdot e^{-\frac{(f-\theta)^2n^2}{Var\cdot r}} \leq t\mbox{ (False Positive Constraint)}\\
\end{align*}

The analysis shows we should use as few phases as possible anyway. Thus the limitation is on the computation power.
We (switch to the top-k definition) want to limit the size of candidates in each phase, which can determine the number of rounds (there is no $\theta$).

Since each initial phases will output $C>k$ candidates, the initial phases can tolerate more undesired errors. Therefore we will have the following questions:
\begin{itemize}
	\item 
	maybe we can use smaller group size in beginning groups, and larger size in the final group
	\item
	longer segment size (more computational power) in initial phases, and a short segment in the final phase
\end{itemize}

As for the hashing based method, 
based on $k$, we have an estimation on the number of channels to use (e.g., $k^{2}$, to guarantee that the collision probability of heavy hitters is small),
then by the computation limit, we also have the segment length and number of rounds. 
Note that there must exists a group of users allocated for testing the full value, since in each channel, we can't get an accurate estimation of the heavy hitter because of collision in each segment from other values.
This is different from the other method where the reports from the last group are based on the full values. How many users should be allocated in the last group, however, is still unknown.
Another question is whether the error correction code is useful or not. We should be able to analyze the performance of ECC though.


Now we turn to top-$k$ definition and analyze again. 
The main challenge for this analysis is that, it is hard to analyze the probability a random variable is sampled to be among the top $k$ values.

The naive solution is to assume  $v_j$, the current value under analysis takes some number $x$, and all other values takes value less than $x$, and summing up all the probabilities. This helps us calculating probability $v_j$ comes out first.
However, this method is computationally infeasible.

We make the following approximations:
\begin{itemize}
	\item 
	The top $k$ values appear with frequencies $1/k$. All other values appear with frequencies basically $0$. We also assume there is no collision among the frequent values. That is, for any segment the algorithm will test, any two frequent values take different patterns.
	The reason for assuming this is that the underlying distribution is unknown, and we believe different distributions will result really no big difference.
	
	\item
	Because of the simplified distribution, we are now safe to say that except the last phase, where exactly $k$ values should be output, all the beginning phases work exactly the same. Therefore, we only have these parameters: $r$ is the number of rounds, $s$ is the step length for each phase, $C$ is the candidate size output by each phase. As a result, the first phase analyze $\log C+s$ bits, the following phases each analyze $s$ bits, except the last phase, which analyzes $m-\log C-s(r-1)$ bits. The last phase also can have $n_r$ users to participate, and all the other phases will thus have $\frac{n-n_r}{r - 1}$ users to report.
	
	\item
	We use normal distribution to approximate binomial distribution whenever it is possible.
	
	\item 
	We assume no correlation among the top few variables. That is, the expected number of top-$k$ values among the $C$ candidates is the summation of each of them among top $C$ after estimation.
	
	\item
	The last approximation is about how to calculate the probability a value is tested to be at a certain rank. We assume all the other values will be sampled following the assumed distribution. Therefore, we know expectedly how many values are above a certain value. For example, in expectation, $y$ values are tested above $x$ (this can be computed basically by the CDF of normal distribution). We already know the distribution of the current value, then we can easily calculate the approximate probability it ranks $y$ (that is, the probability it takes value $x$).
	
\end{itemize}
\begin{align*}
\mbox{input: }
& n\mbox{ is number of users}\\
&\epsilon\mbox{ as privacy budget and } p=\frac{1}{2}, q=\frac{1}{e^\epsilon+1}\\
&m\mbox{ is total length of binary representation of input}\\
&f_j\mbox{ is the frequency of the $k$-th most frequent value}\\
%&\{f_1,f_2,\ldots,f_{2^m}\}\mbox{ is the dataset distribution s.t., } f_1=f_2=\ldots=f_{k}=\frac{1}{k} \mbox{ and } \sum_{j=1}^{2^m}f_j=1\\
&k\mbox{ is the size of the output }\\
&p\mbox{ is the computational power limit}\\
\mbox{choose: }
& r \in\mathbb{Z^+}\mbox{ is the number of phases}\\
&\forall i\in\{1,2,\ldots,r\}\\
&\;\;\;\;\;\; C_i=C \mbox{ is the size of candidates to output in each initial phase}\\
&\;\;\;\;\;\;\;\;\;\;\;\;\mbox{for the last phase, } C_r=k\\
&\;\;\;\;\;\; s_i=s_1 \mbox{ is the step length for each initial phase}\\
&\;\;\;\;\;\;\;\;\;\;\;\;\mbox{s.t., for the last phase, } s_r=m-\lceil\log_2C\rceil-s_1\cdot (r-1)\\
&\;\;\;\;\;\; n_i=n_1 \mbox{ is the number of users in the each initial phase}\\
&\;\;\;\;\;\;\;\;\;\;\;\;\mbox{s.t., for the last phase, } n_r=n-n_1\cdot(r-1)\\
\mbox{subject to: }
&(2^{s_1}\cdot (r-1)+2^{s_r})\cdot C < p\mbox{ computation power limit}\\
\mbox{maximize: }& \etp=\sum_{j=1}^{k}\left(\prod_{i=1}^{r}\Pall{j}{i}\right)\\
\mbox{where: }
%&\forall i\in\{1,2,\ldots,r\}, \forall j\in\{1,2\ldots,k\}:\\
%&\;\;\;\;\;\;\Pall{j}{i}=F\left(C_i-j;2^{s_i},1-\Phi\left(\frac{ n_i(\delta_i(p-q)-q)-\mu_i[j]}{\sigma_i[j]}\right)\right)\\
&\Pall{j}{i}=1 - \Phi\left(\frac{ \Phi^{-1}\left(\frac{C_i-j}{2^{s_i}-j}\right)\sigma_i[0]+\mu_i[0]-\mu_i[j]}{\sigma_i[j]}\right)\mbox{ (when $C_i>j$)}\\
%&\;\;\;\;\;\;\\
\end{align*}
To compute \Pall{j}{i}, we first assume all other $2^{s_i}$ values take zero probability. Since they each follows a normal (binomial) distribution, we can compute $x$, such that expectedly $C_i-j$ values are among $x$ (basically by inverse cdf of the normal distribution). Then we compute the probability the current value is above the fixed value $x$. This is the expected value it advances to the next phase.

There seems no available optimizers for this problem. However, it is fortunate the number of optimizations that need to be searched for is limited. We start from an initial configuration, and vary parameters (the three parameters $r, C, s_1$ are related to each other given the computation power limit) to get different configurations. The parameter for the number of users, $n_1$ can have multiple choices (around $n$) and is independent on the other parameters. However, we can have larger steps.
Another observation is that it is better to use up all the computational power.

Because of the computation constraint, we start 
The first configuration we start with is assume
\begin{comment}
\subsection{Optimal Configurations}
We have analyzed the identification probability of candidates in each group, and the final probability is that to the power of the number of groups. While these analysis match empirical results, it is not optimal. Finding optimal parameters for the protocols, i.e., what is the segment length, and what branching factor should we choose.

\mypara{Optimal Segment Length.}
Without considering the constraint of computational power, larger segment size will decrease number of groups, which result the increase of probability a true heavy hitter is identified. However, more false positives will also be produced. As a result, the optimal segment size is dependent on the threshold and privacy budget.

We choose to analyze and \itergroup for simplicity. Note that \product can also be analyzed, but the tree structure makes it less flexible (although it is more paralleled). 

For a given privacy budget and threshold, the optimal choice of segment size can be modeled as an optimization problem:
\begin{align*}
\mbox{optimize: }& \mbox{f1 score}\\
\mbox{subject to: }& s \geq 1\\
				& s' = s - \log_2\left(\EV{TP}+\EV{FP}\right)
\end{align*}

By Theorem~\ref{thm:group_eq_size}, each group has the same amount of users. Analyzing the first segment will result some candidates. With that, we can analyze further segments. As we move forward, we may only have very few non-heavy hitters with high frequency (we assume they have zero frequency), and based on that, we can calculate the expected false positives.
Analytical results are given in Figure~\ref{fig:opt_s}.

\mypara{Optimal Group Size.}
We use the same group size in all groups. Now we show this is the optimal choice.
Recall a candidate with probability $f$ is identified by threshold $T$ is $P_0^g=\left(1-F(T;n_s,fp+(1-f)q)\right)^g$. $P_0$ (and thus $P_0^g$) is concave when $fn_s>T$, therefore, by Jensen's inequality, use the same size for each group will result the optimal summation of probabilities in each group, which corresponds to the optimal overall probability, which is the product of these probabilities.

\mypara{Optimal Structure.}
Having segment length fixed, the branching factor $b$ for \product should be set to be $\log_{\EV{TP+FP}}2^s$.
\says{tianhao}{this becomes a complicated formula, but we can solve it by just enumerating.}

For \itergroup, we can set up which segment one needs to report in advance, this brings some more flexibility. Specifically, given initial $s$, we are able to approximate the expected candidates that can be identified, then the next test can cover an additional $s-\log_2\EV{TP+FP}$. This analysis can even be adaptive.

\mypara{Corner Case Handling.}
Since the structures are not fine-grained, we need to handle corner cases. 
In \product, when we cannot build a complete binary tree, we combine the nodes bottom up.

\itergroup has the problem that the final group don't need to handle a full segment. One can just let the final group handle the segment left, or partition the rest of the segments evenly into the rest of groups.
\end{comment}
\begin{comment}
Next, we measure precision, namely $FP/(TP+FP)$ for different segment length. We fix a threshold, and count how many values can be reliably identified (with probability greater than $90\%$), versus expected number of values that does not belong to the top $k$ hitters but will be identified in \textbf{one} segment.

We plot the results in Figure~\ref{fig:fix_T}. As we can see from the figures, when the threshold increases, the precision increases, this is because the increased threshold will result decrease of reliable true positives, but also decrease of expected false positives in one segment. This guides us to choose a threshold so that we can reliably identify as many values as possible, while not bringing too many false positives.


Similar to Figure~\ref{fig:fix_k}, in Figure~\ref{fig:vary_T}, we fix a threshold, and then calculate the relationship between expected number of true positives and false positives, i.e., $\EV{TP}, \EV{FP}$. A value with frequency greater than $T$ and tested to be with frequency above $T$ is taken as a true positive, and a value with frequency lower than $T$ but tested to be with frequency above $T$ in \textbf{any} segment is taken as a false positive. We plot $\EV{TP}$ versus $\frac{\EV{TP}}{\EV{TP}+\EV{FP}}$. When the ratio is still high (e.g., above $50\%$), we can take the $x$ value of the point as the expected number of heavy hitters that can be identified, and we expect to tolerate $\frac{1}{y}-1$ fraction of errors. As we can see in the figures, for different segment sizes, we can recover different number of heavy hitters, without affecting the overall performance badly. 

The intuition behind Figure~\ref{fig:vary_T} is that, the probability a value is identified in one segment is fixed, given $T$ and $f$. Fixing $T$, varying $f$, the probability $p$ is actually the CDF. On the other hand, the probability a value is identified as a heavy hitter is $p^g$, since it should be identified in all groups. On the one hand, we want to identify as many heavy hitters as possible; on the other hand, we don't want to introduce too many false positives. Therefore, we want to maximize expected true positives while minimize false positives.

The expected values can be visually seen in Figure~\ref{fig:cdfs}. 

\says{tianhao}{to be tested}
One property is that, varying T does not affect the horizontal distance between the two curves. This is because the right curve is determined by the left curve, and by the property of Normal (Binomial ) distribution, the shape (slope) does not change. 
\end{comment}

%\input{norm_inv.tex}

\begin{comment}
\subsubsection{Effect of Error Correction Code}
Now we analyze the effect of error correction code, by compare the probabilities of identifying a heavy hitter of some frequency $f$ in two protocols: \hash and \hash with error correction code.


For \olh and \oue ($s>1$), similar to the case when $s=1$, we have $q'=\frac{1}{2^s}p+\frac{2^s-1}{2^s}q=q+\frac{1}{2^s}(p-q)$.

Therefore, firstly, the variance is not optimal for this setting, secondly, the significant test should be adjusted to $q'$ instead of $q$.
\\
Suppose only the heavy hitter under analysis is hashed into this channel (this probability of collision is only dependent on the channel size) and no other candidates is hashed into this channel.

\textbf{General Analysis.}
Similar as our analysis in Equation~\ref{eq:single}, now we analyze probability a heavy hitter is identified. We first parameterize out some constants into the following Equation:

\begin{align}
p(N,T,p,q)=&\sum_{n_f=0}^{N}\Pr{n_f|n,f}
		\sum_{n_1=0}^{n_f}\Pr{n_1|n_f,p}
		\sum_{n_2=T-n_1}^{N-n_f}\Pr{n_2|N-n_f,q}\label{eq:hash1}
\end{align}

The event a heavy hitter is identified in a segment can be dissected into three sub-events:
\begin{itemize}
	\item $n_f$ users are assigned into this segment.
	\item For this segment, $n_1$ out of the $n_f$ users report faithfully.
	\item Among the other $n_s-n_f$ users, $n_2$ users contribute, such that $n_1+n_2$ is above a threshold.
\end{itemize} 


For the setting of $s=1$, there are only two possibilities. Thus we can use the random response method \DE (it is also possible to use \olh or \oue, but they result in a $p=1/2$, whereas $p=\frac{e^\epsilon}{e^\epsilon+1}$ in \DE).

\textbf{Background on Coding Theory.}
Coding theory is used in the noisy channel where messages are transmitted with some errors. In the current setting, therefore, we can use encoding and decoding systems to correct possible errors.

In the coding scenario, a message of length $m$ will be encoded into a message of length $m'$. The rate of the code is $\frac{m}{m'}$. A typical unique code (Reed-Solomon~\cite{reed1960polynomial}) will correct approximately $\frac{1-R}{2}$ fraction of errors, while a simple list decoding (improved list decoding of Reed-Solomon~\cite{sudan1997decoding}) can correct $1-\sqrt{R}$ fraction of errors. The optimal list decoding (folded Reed-Solomon codes~\cite{guruswami2008explicit}) can correct $1-R$ fraction of errors, but it requires $m'$ to be large, and it takes longer time than the simpler ones.

\textbf{Specific Analysis.}
Now we analyze the probability in different settings:


\begin{itemize}
	\item No ECC: 
	\[
	p_s=p(N=n/m,T=\sqrt{ns/m\frac{1}{e^\epsilon -1}},p=\frac{e^\epsilon}{e^\epsilon+1},q=\frac{1}{e^\epsilon+1})
	\]
	\[
	\Pr{Iden}=p_s^m
	\]
	We can tolerate some errors (i.e., $2$) in some segments, thus 
	\[
	\Pr{Iden}=\sum_{s_i=m-2}^{m}\Pr{s_i|m,p_s}
	\]
	\item Naive optimal ECC from $m$ to $m'$: Naive unique ECC will extend the message from $m$ bits to $m'=m/R$ bits, where $R$ is the rate of the code. The optimal unique ECC can correct asymptotically $\frac{m'-m}{2}$ errors. Therefore,
	\[
	p_s=p(N=n/m',T=\sqrt{ns/m'\frac{1}{e^\epsilon -1}},p=\frac{e^\epsilon}{e^\epsilon+1},q=\frac{1}{e^\epsilon+1})
	\]
	\[
	\Pr{Iden}=\sum_{s_i=m+(m'-m)/2}^{m'}\Pr{s_i|m,p_s}
	\]
	Assuming $m'=1.5m$, the overall probability is higher. But if $m'=2m$, the overall probability is lower.
	\item Naive optimal list decoding ECC from $m$ to $m'$: List decoding can handler more errors by outputting a list of messages instead of one in unique ECC. State of the art list decoding schemes can correct all the redundant bits.
	Therefore,
	\[
	p_s=p(N=n/m',T=\sqrt{ns/m'\frac{1}{e^\epsilon -1}},p=\frac{e^\epsilon}{e^\epsilon+1},q=\frac{1}{e^\epsilon+1})
	\]
	\[
	\Pr{Iden}=\sum_{s_i=m}^{m'}\Pr{s_i|m,p_s}
	\]
	\item Optimal list decoding ECC from $m$ to $m'$, with overall significance:
	Suggested by Bassily and Smith~\cite{Bassily2015local}, the criteria for picking a candidate in a segment does not rely on the threshold, but the top one. After the list decoding, they filter out the false positives by calculating whether the overall frequency is above a threshold.
	This is not easy to model by probabilities, we use the above analysis to approximate.


\end{itemize}



For hash based methods, we use $1/2^s$ instead of $q$ in Equation~\ref{eq:single}, because every user with other values (not hashed into this channel) should report uniformly.


For each position, the value can be regarded as the summation of two binomial distributions: for those with $1$ in the first layer, the true value appears with probability $p$, and for a $0$, a random value is reported.

No error correction: $p(m)^m$.
With error correction: encode $m$ to $m'$ bits, thus when $l$ out of $m'$ bits are correct, we can identify the correct answer: $\sum_{c=l}^{m'}{{m'}\choose{c}}p(m')^c(1-p(m'))^{m'-c}$




For \hash with larger segment size, i.e., \simhash, recall that we use a threshold to select candidates. However, when $s=1$, there are only two possible candidates, thus it is enough to pick the one with more occurrence (the candidate with more occurrence is taken in the original protocol of \hash as well).

Note that it is also possible to apply error correction code in the case where a larger alphabet is used (i.e., $\Sigma=\{0,1,\ldots,2^s-1\}$). We can also estimate the effect of error correction code in that case. But when $s>1$, we can only analyze using a threshold, since it is not easy to estimate the frequency for ``a candidate occurs the most frequently''. 

It is possible to also use a threshold to determine if the detected candidate is reliable, therefore reduce false positives. 
If the significant test is used, we can therefore determine if an identified candidate is significant, and thus if no candidate is significant for a segment, we can enumerate all possibilities or the highest few in that segment. However, this does not work when most of the segments are not significant, making the task computationally infeasible.
\end{comment}





%The motivation behind coding theory is that, the noisy channel transmits each bit correctly with a fixed probability. However, here, the more bits used to transfer, the lower each bit can be correctly transmitted. It is unclear whether using coding theory here is a good strategy or not.
\begin{comment}
Specifically, assume the users are assigned to each position randomly (for each position, there are $n/\log d$ users, where $\log d$ is bit vector length, and a ratio $f$ of them have true value), what is the probability the current bit is correctly recovered?

What the aggregator sees is a combination of two binomial distributions $Binom(nf/\log d, p)$ and $Binom(n(1-f)/\log d, 1/2)$. 
By Chernoff bound, the probability an error (aggregated bit is different) occur with exponential probability:

\begin{align*}
&\Pr{X-nq/\log d \leq 0} = \Pr{X\leq nq/\log d}\\
= &\Pr{X\leq npf/\log d+n(1-f)/2\log d+}\\
\leq &A^{n/\log d}
\end{align*}


(assume the current value under test is a heavy hitter, and no collision happens). 
Thus, probability the recovered bit vector is correct is $(1-A^{n/\log d})^{\log d}$.

On the other hand, if more bits are tested with error correction, for each bit, we have probability $A^{Rn/\log d}$, where $R\in[0,1]$ is the rate of the code, (by the same assumption).
Because of the error correction code used,
a $\tau\in[0,1]$ fraction of errors can be tolerated, 
thus, the overall error probability is 
\[
\sum_{i=(1-\tau)\log d/R}^{\log d/R}{{\log d/R}\choose{i}}(1-A^{Rn/\log d})^{i}(A^{Rn/\log d})^{\log d/R-i}
\]
\end{comment}
%\mypara{Utility Analysis of \rappor.}

\input{table_compare_ana.tex}
%
%
%. (\textit{Assumption 1:}) We use Normal distribution to approximate how many users with heavy hitter are assigned to a specific segment. The Normal distribution has mean $nf/g$ and variance $nf\cdot\frac{1}{g}\cdot\frac{g-1}{g}$. (\textit{Assumption 2:}) Assume for simplicity users with other values all have different values in this segment. We can calculate the probability $n'f'$ out of $n'=n/g$ users have the heavy hitter in this segment:
%
%\begin{align*}
%\Pr{n'f'}^1&=f(n'f'|n'f,n'f\frac{g-1}{g^2})\\
%&=\frac{g}{\sqrt{2n'f(g-1)\pi}}e^{-\frac{n'(gf'-gf)^2}{2f(g-1)}}
%\end{align*}
%
%With $n'f'$ heavy hitters, now let's calculate what is the probability it is identified in the current segment. (\textit{Assumption 3:}) For simplicity, we calculate the probability the recovered heavy hitter is above some threshold.
%
%\begin{align*}
%\Pr{n'\tilde{f'}\geq T}^2&=1-\Phi\left(\frac{\Phi^{-1}\left(1-\frac{1}{20\cdot 2^s}\right) \sqrt{\sigma^2\cdot n'}-n'f}{\sigma\sqrt{n'}}\right)\\
%&=1-\Phi\left(\Phi^{-1}\left(1-\frac{1}{20\cdot 2^s}\right) -\sqrt{ns/m}f/\sigma\right)
%\end{align*}
%
%
%
%The probability a heavy hitter is identified in one segment is:
% 
%\begin{align*}
%\Pr{f}^{node}&=\sum_{n'f'=0}^{n'}\Pr{n'f'}^1 \Pr{n'\tilde{f'}\geq T}^2
%\end{align*}
%
%\mypara{Put it together.}
%(\textit{Assumption 4:}) Assume all segments are independent. The overall probability a heavy hitter is identified is:
%\begin{align*}
%\Pr{f}=\prod_{node}\Pr{f}^{node}
%\end{align*}



\subsection{Empirical Result}
Now we perform experimental evaluation to confirm that the analysis matches the empirical results. We generate a set of $1$ million and $10$ million strings of length $64$ and $256$, respectively, following a Zipf's distribution (specifically, $\Pr{X=i}\propto\frac{1}{(i+20)^{1.5}}$). All experiment runs in ten rounds.

\input{all_figures.tex}


%\mypara{On Privacy Budget.}
%Increasing privacy budget helps recovering more heavy hitters. In Figures~\ref{fig:pri_count} and~\ref{fig:pri_prob}, we show the total number of heavy hitters identified, and the probability a heavy hitter with a fixed original probability is recovered, respectively. Results in Figure~\ref{fig:pri_prob} are get from $200$ runs.

\mypara{On Number of Channels.}
In the hash based methods, increasing the channel size will decrease the probability that different candidates collide in the same channel, thus increase the total amount of candidates identified. 
However, as shown in Figures~\ref{fig:channel_count} and \ref{fig:channel_stat}, after a threshold, increasing the number of channels does not help, this is because the collision probability is already low enough that basically no heavy hitters are hashed into the same channel. On the other hand, the computational overhead is too much that we skip those points.


\mypara{On Identification Probability.}
Figures~\ref{fig:comp_1000000} and~\ref{fig:comp_10000000} show the probabilities values with different frequencies are identified. Analysis matches empirical results.

\mypara{On Expected Identified Candidates.}
Figures~\ref{fig:emp} shows the number of values that can be identified.\says{tianhao}{should calculate expected value}

\mypara{On optimization efforts of a simplified problem.}
Figures~\ref{fig:simple_opt} shows the expected \fone score for different $s$ values.

\mypara{On top-k problem.}
We examine the ``top-k'' problem here (Definition~\ref{def:topk}). In this setting,
the goal is to find out the top $k$ heavy hitters. However, each phase will output $\alpha k$ values, where $\alpha$ is a multiplicative factor whose effect we want to test.
An additional $s$-bit segment is analyzed in each phase, except that the first phase handles $s+\log\left(\alpha k\right)$ bits, and the last phase handles whatever is left.
Table~\ref{table:com} give numerical results when $\alpha=1, s=8$ and $k=256$.
Figures~\ref{fig:T_vary_8} and \ref{fig:T_vary_12} shows the averaged \fone score varying $\alpha$ for different $k$ values. 

\mypara{Problems to be Solved.}
ECC will help for hashing based method. What is the optimal ECC code? Will the optimal ECC configuration outperform \itergroup or \product?



\mypara{Potential Optimizations.}
One idea of improvement is to check for missing candidate after each layer. For instance, if in some phase, the total frequency of all identified values is still small, there might be some frequent values missed in the current or previous phases. In this case, some backoff methods to find the missing values might be desired.


\begin{comment}
	

Here are the list of experiments we are expected to show. 

\begin{enumerate}
	\item Optimal configurations of different methods. Assuming each user reports one or two bytes ($8$ or $16$ bits).
	
	\begin{itemize}
		\item First of all, we show by experiment that partitioning the population is better than dividing the privacy budget. \says{tianhao}{todo}
		\item 
		
		
		\mypara{On number of channels.}
		Given the number of users $\sqrt{n}$, there's an upper bound on the number of domains that can be precisely estimated (i.e., those with count higher than $\Phi^{-1}\left(1-\frac{0.05}{d}\right) \sqrt{\sigma^2\cdot n}$, where $\Phi$ is the inverse of standard normal cdf, and $\sigma^2$ is the variance). In that sense, we need $\sqrt{n}^{t}$ instead of $n^{t}$ in order to minimize the collision of heavy hitters. Moreover, if the distribution is not uniform, the test can be much less.
		% seems the following analysis is wrong
		
		%\mypara{Discussion 1. Optimality of the Underlying Primitive.}
		%The protocol satisfies $\epsilon$-LDP because of the properties that each user only reports his true value (with perturbation) once. This is in fact a two level encoding: the first layer is a unary encoding (where the user input is $1$ when his value hashes to that slot, and $0$ otherwise); the second layer is a coding encoding, where each user (if his first layer input is $1$ for that slot) randomly select a position, and then report the bit at the position of the coding of his true value. 
		%We can transmit more information by encoding the first layer using OUE.
		%
		
		\item How many errors should we tolerate? \says{Tianhao}{should discuss in description.} The more we tolerate, the more true positives there will be, but the false positives also grow exponentially.
		\item Optimal branching factor? It is intuitive to use constant branching factor, but it is possible to adaptively choose the branching factor and get better result. \says{tianhao}{maybe we could analyze this theoretically and ignore this so-complicated experiment here.}
	\end{itemize}
	
	\item Comparison of different methods, using similar amount of computation. We assume the client-side computation and network communication are not bottleneck of all the protocols (although they are quite different for different methods).
	
	\item We also show the effectiveness of existing methods.
\end{enumerate}
\end{comment}

\begin{figure*}[t]
	\centering
	\subfigure[Vary \# Channels, \# Heavy Hitters Identified]{
		\label{fig:channel_count}
		\includegraphics[width=0.45\columnwidth]{figure/vary_hash_len_count}
	}
	\subfigure[Vary \# Channels, Total True Count Heavy Hitters Identified]{
		\label{fig:channel_stat}
		\includegraphics[width=0.45\columnwidth]{figure/vary_hash_len_stat}
	}
	\caption{Effect of the number of channels in identifying heavy hitters. We show the number of heavy hitters identified (Figure~\ref{fig:channel_count}), and their true count (Figure~\ref{fig:channel_stat}) varying the channel size, for different segment length ($4, 8, 16$ bits). For $1$ and $2$ bits, basically zero heavy hitters can be identified, so we ignore them in these figures.}
	\label{fig:cmp_dist}
\end{figure*}

\begin{figure*}[t]
	\centering
	\subfigure[$s=8$]{
		\label{fig:T_vary_8}
		\includegraphics[width=0.45\columnwidth]{figure/T_alpha/n100000m64e4s8}
	}
	\subfigure[$s=12$]{
		\label{fig:T_vary_12}
		\includegraphics[width=0.45\columnwidth]{figure/T_alpha/n100000m64e4s12}
	}
	\caption{\fone score for different $k$ values varying $\alpha$. We use $n=100000$ users.}
	\label{fig:T_vary}
\end{figure*}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% use &\tabincell{c}{}& for new lines in a table cell
\input{table_compare_all.tex}

\begin{comment}
\subsection{How to Choose Parameters.}
\says{tianhao}{maybe delete this section.}
Given the fact that it is better to partition the population, a natural research question is how to partition the population. On the one hand, it is not realistic to let users send too much information (e.g., more than mega-bytes), and the computation on the server side should also be feasible. On the other hand, by letting each user report more information and server do more computation, the utility can definitely improve. An extreme example is to let each user report his full value, which acts as an optimal baseline, but it is not computationally feasible.

Now we analyze the optimal way to partition the population in each protocol we proposed.

Suppose the values are represented by bits, and each user has a value of length $m$. The problem is to find the optimal value $s$, the length of the segment each user reports. 

Given $s$ and $m$, there are $m/s$ different non-overlapping segments. Thus we have at most $s\cdot n/m$ users for each segment.

Note that all LDP primitives (except Random Response-based protocol, which is not accurate) require $O(n\cdot d)$ computation time, where $d=2^m$ is the domain size. If we split the population into $m/s$ groups, the overall computation time is $O(\frac{ns}{m}\cdot 2^s\cdot m/s)=O(n\cdot 2^s)$. Thus, the more fine-grained we split the domain, the more efficient the protocol is (but also less accurate).

To make a fair comparison, it is desired to require every protocol to be compared run in a similar time complexity. Suppose $\alpha$ hash functions are used, \simhash runs in $O(\alpha n \cdot 2^{s'})$ time; \product runs in $O(\frac{n}{2t}\cdot 2^s\cdot 2t)=O(n\cdot 2^s)$ time; \itergroup runs in $O(n\cdot 2^s)$ time. Conceptually, $\log\alpha$ more bits is required for \simhash, i.e., $s'+\log\alpha=s$.

\mypara{Optimal Branching Factor}
We assumed the branching factor to be $2$ for the \product protocol. But what is the optimal branching factor? For the fairness and simplicity of the protocol, we assume each node the server handles the similar amount of users in each node, with a similar amount of computation.
Suppose the branching factor is $b$. There are $m/s$ nodes in the last layer, and there are $\frac{m/s\cdot b - 1}{b - 1}$ nodes in the whole tree. 
By the previous analysis, $\sqrt{cn'}$ candidates can be identified on average, where $c$ is a constant typically within $[2,4]$, and $n'=n / \frac{m/s\cdot b - 1}{b - 1}$. An optimal configuration would require each node have the same domain size as input, thus
\begin{align*}
&\left(\sqrt{\frac{cn(b - 1)}{m/s\cdot b - 1}}\right)^b\simeq 2^s\\
\implies &b\cdot\log\frac{b-1}{b}\simeq \frac{2s}{\log \frac{cns}{m}}
\end{align*}
If we concrete the parameters $n=10^6, m=256, s=16$, $b=2$ will achieve this equation.

\mypara{Comparison between \simhash and \product}
To summarize, we effectively improve the running time of the protocol from $O(n\cdot 2^m)$ to $O(n\cdot 2^s)$,
(to $O(n\cdot 2^{(s'+h)})$ for \simhash) but we can detect candidates with frequency higher than $\sqrt{cn\cdot\frac{2m}{s}}$ ($\sqrt{cn\cdot\frac{m}{s'}}$ for \simhash).

In order to make the comparison fair enough, all protocols should use the same amount of time, thus the two protocols are equivalent if $h=s'$. The disadvantage of \simhash is that two heavy hitters may collide in the same hash function; the advantage is that no additional information of partial heavy hitters is leaked to the users.

\mypara{Comparison between \itergroup and \product}
For the \itergroup protocol, if we use the same $s$ value as in the \product protocol, the domain size would be too big. So we should use a smaller $s'$ such that 
\begin{align}
&\left(\sqrt{\frac{cns'}{m}}\right)\cdot 2^{s'} \simeq 2^s\label{eq:iter_prod}\\
\implies&\log\left(\sqrt{\frac{cns'}{m}}\right) \simeq s - s'\nonumber
\end{align}
With the same amount of computation, we can detect candidates with frequency higher than $\sqrt{cn\cdot\frac{2m}{s}}$ ($\sqrt{cn\cdot\frac{m}{s'}}$ for \itergroup).
Thus, the two protocols achieves similar accuracy when $s=2s'$.
Fixing parameters $n=10^6, m=256, s=16$, and $c=2$, LHS of Equation~\ref{eq:iter_prod} is smaller than RHS, which means \itergroup requires less computation power than \product.

\end{comment}

%With more redundancy, more 

\input{fix_figures.tex}

==> cot.tex <==
\subsection{\cot Data Structure}
\label{subsec:cot}

==> covt.tex <==
\subsection{The \covt Data Structure}
\label{subsec:covt}

A \covt is a labeled tree where each node $u$ is given a label $L(u)\subseteq\{1,2,\ldots,m\}$, 
where $m$ is the length of the binary representation of any value in the domain $D$, i.e., $m=\log_2 |D|$.

There are exactly $m$ leaf nodes in \covt and each leaf node is labeled with exactly one distinct element from $1$ to $m$,
corresponding to one index of the domain value.
For each non-leaf node, its label is the union of the labels of its children.
%Labels of any two nodes do not intersect if they are not in the same path (one is not ancestor of the other).
The label of the root node is $\{1,2,\ldots,m\}$.
Any leaf node is covered by some internal nodes.
We thus call it \covt.
Figure~\ref{fig:protocols_trees} shows two examples of \covt.
%Any leaf node represented by the gray box is covered by some internal nodes as blue circles.
%Therefore, we call it \covt.
%We will explain the details of these figures in the following sections.


\begin{figure}[t]
	\centering
	\subfigure[\covt for \product]{
		\label{subfig:hie_tree}
		\includegraphics[width=0.4\columnwidth]{figure/prod_tree}
	}
	\subfigure[\covt for \itergroup]{
		\label{subfig:iter_tree}
		\includegraphics[width=0.4\columnwidth]{figure/iter_tree}
	}
	\caption{\covt for \product and \itergroup. Leaf nodes are represented by gray boxes, and are covered by internal nodes shown as blue round rectangles.}
	\label{fig:protocols_trees}
\end{figure}

Given a \covt, now we construct an LDP protocol.
\begin{algorithm}
	\caption{Aggregator's algorithm to find out top $k$ values.}\label{alg:covt_server}
	\begin{algorithmic}[1]
		\Require \covt, $Y$, reports from $n$ users.
		\Ensure $k$ values.
		\Procedure{Find}{\covt, $Y$}
		%			\State $nn\leftarrow$ number of non-leaf nodes in \covt.
		%			\For{each non-leaf node $u\in\covt$}
		%				\State Sample $n/nn$ users without replacement.
		%				\State Send $L(u)$ to these users.
		%			\EndFor

		\State Initiate candidate set $C(l)=\{0,1\}$ to each leaf $l$.
%		\For{$i=1$ to $r$}
%		\EndFor
		%			\State Initiate $D(u)=$ to each leaf node $u$.
		\State Topo-sort non-leaf node into $u[1],u[2],\ldots,u[r]$.
		\For{$i=1$ to $r$}
			\State Initiate domain set $D(u[i])=\emptyset$.
			\For{$uc\in$ $u[i].children$}
				\State $D(u[i])= D(u[i])\times C(uc)$\Comment{Cartesian product.}
			\EndFor
			\State Receive $Y(u[i])$, reports on $u[i]$.
			\State Feed $Y(u[i])$ to the frequency oracle.
			\State Query the oracle about each value in $D(u[i])$.
			\State Assign top $k[i]$ estimated values to $C(u[i])$.
		\EndFor
		\State \textbf{return} $C(u[r])$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
The analyzing task for the aggregator is presented in Algorithm~\ref{alg:covt_server}.
It takes a public \covt, and $n$ reports $Y$, and returns $k$ values.
Suppose that \covt has $r$ non-leaf nodes (node for short), and $m$ leaves.
Within the algorithm, 
there is a default candidate set $\{0,1\}$ associated with each leaf.
For each node $u[i]$, and two associated sets,
i.e., a domain set $D(u[i])$, and a candidate set $C(u[i])$.
The domain set is the set of values that will be queried to the frequency oracle.
It is constructed as a Cartesian product of candidate sets from its children.
The frequency oracle takes in $n[i]$ reports, $Y(u[i])$,
where $n[i]$ is the number of users who choose node $u[i]$,
and estimate frequencies for values in $D(u[i])$.
After the estimation, the aggregator takes $k[i]$ values with the most estimated frequencies as the candidate set.

Overall, the aggregator sorts the nodes topologically, 
and for each node $u[i]$, he constructs the domain set $D(u[i])$ and works out the candidate set $C(u[i])$.
The same operation is performed repeatedly until the $C(u[r])$, the candidate set for the root node, is returned as the final result.

From the user's perspective,
each user $j$ chooses one node $u[i]$ from \covt uniformly at random.
The user then truncates his value string $v^j$ into a substring $v^j_{L(u[i])}$, 
which is the concatenation of bits whose locations are specified by the label of $u[i]$, $L(u[i])$.
Finally the user sends a tuple $\langle i, y^j\rangle$, 
specifying the node he chooses and the report of his private value purturbed by \olh, i.e., $y^j=\mathsf{P}(v^j_{L(u[i])})$.
%of his substring 
%(perturbed by \olh to satisfy LDP).


In the example of Figure~\ref{subfig:iter_tree},
the non-leaf nodes are sorted from left to right.
If a user has value `1101', and chooses the middle node $u[2]$,
he uses \olh to report value `110'.

The aggregator works on $u[1], u[2], u[3]$ one by one.
Firstly, $D(u[1])=\{0,1\}\times\{0,1\}=\{00,01,10,11\}$ is constructed.
The aggregator then collects reports for $u[1]$ and gives the reports to the frequency oracle.
The frequency oracle estimates the frequencies of all values from $D(u[1])$,
and the two with higher frequencies (suppose they are $10,01$) are assigned to $C(u[1])$.
For $u[2]$, its domain set $D(u[2])=C(u[1])\times\{0,1\}=\{100, 101, 010, 011\}$.
The aggregator repeats the same operation as for $u[1]$ until the root node,
whose candidate set can be returned as the result.
%For instance, if the user receives $\{1,3,4\}$, he will truncate his value into a three-bit (i.e., bit 1,3,and 4) string.

%starts from one non-leaf node, 
%which means to examine a small segment, and find out frequent patterns for this segment.
%The frequent patterns is then sent to the parent node, 
%and this analyzing and finding operation is repeated.
%Similar to \spm, 
%the intuition is that if a value is frequent in a larger segment,
%parts of it must be frequent in a smaller segment.
%Different from \spm, 
%the segments are extended or combined,
%so that the final result is given in the whole segment,
%thus minimizing the number of tests.

%Specifically, protocols following \covt work as follows:
%Each user is assigned to one non-leaf node in \covt; the label of the node is sent to the user.
%The user uses \olh to report a substring of his private value. The substring is selected using the indices specified by the label.
%For instance, if the user receives $\{1,3,4\}$, he will truncate his value into a three-bit (i.e., bit 1,3,and 4) string.
%
%From the server's perspective,
%the identification process works in a topological order:
%Without considering the leaves from \covt, the aggregator starts from nodes without children.
%Then it proceeds with the nodes whose children are all ready.
%In the example of Figure~\ref{subfig:iter_tree}, 
%the aggregator starts from the node with label $1,2$, then $1,2,3$, and finally $1,2,3,4$.

%The aggregator makes each node ready by querying the frequency oracle of all possible values,
%referred as intermediate domain,
%and finds out the ones in the intermediate domain that are frequent, 
%referred as intermediate result.
%The intermediate domain of each non-leaf node is the set of values whose parts are frequent 
%(in the intermediate result) from its children.
%The frequent values of the leaf node are all possibilities.
%For the node with label $1,2,3$ in Figure~\ref{subfig:iter_tree},
%the intermediate domain is the set of values with three bits.
%The first two bits are from intermediate result by the node with label $1,2$, 
%and the third one comes from the leaf node with label $3$, 
%which is basically all possible alphabets 
%(in the case of binary representation, the alphabets are $0$ and $1$).
%The frequent three-bit values are identified as intermediate result and fed to the root node.
%Finally, the result from the root node is the set of final heavy hitters.


%Examples in Figure~\ref{fig:protocols_trees} have domains of four bits, i.e.,
%$L(D)=\{1,2,3,4\}$. 
%In Subfigure~\ref{subfig:hie_tree},
%two internal nodes with labels $\{1,2\}$ and $\{3,4\}$ cover the four leaf nodes,
%and the root node finally covers these two nodes.
%During analysis,
%the frequent patterns for two bits are found (can potentially be performed parallel) first,
%and then used for the final process,
%which covers the whole domain.
%In Subfigure~\ref{subfig:iter_tree},
%there are three non-leaf nodes,
%labeled $\{1,2\},\{1,2,3\},\{1,2,3,4\}$ respectively.
%During analysis,
%the frequent patterns for two bits are found first,
%and then used in the next phase,
%which covers and finds out frequent patterns in the first three bits.
%Finally, the root node represents the last phase and finds frequent patterns in the whole domain $L(D)$.

%\begin{algorithm}
%	\SetAlgoLined
%	\KwResult{Write here the result }
%	initialization\;
%	\While{While condition}{
%		instructions\;
%		\eIf{condition}{
%			instructions1\;
%			instructions2\;
%		}{
%			instructions3\;
%		}
%	}
%	\caption{How to write algorithms}
%\end{algorithm}

%\begin{algorithm}
%	\caption{Our Proposed Standard SVT}
%	\label{alg:standard}
%	\begin{algorithmic}[1]
%		\Require $D,Q,\Delta,\mathbf{T}=T_1,T_2,\cdots,c$ and $\epsilon_1, \epsilon_2$ and $\epsilon_3$.
%		%, allocated to  the threshold, to query answers for determining whether each query is above the threshold or not and to above query answers for numeric outputs, respectively.
%		\Ensure A stream of answers $a_1, a_2, \cdots$
%		\State $\rho = \Lap{\frac{\Delta}{\epsilon_1}}$, count = 0
%		\For {Each query $q_i \in Q$}
%		\State $\nu_i = \Lap{\frac{2c\Delta}{ \epsilon_2}}$
%		\If{$q_i(D)+\nu_i \ge T_{i} + \rho$}
%		\If{$\epsilon_3 >0$}
%		%\STATE $\gamma_i = \Lap{\frac{c\Delta}{\epsilon_3}}$
%		\State \textbf{Output} $a_i = q_i(D)+\Lap{\frac{c\Delta}{\epsilon_3}}$
%		\Else
%		\State \textbf{Output} $a_i = \top$
%		\EndIf
%		\State count = count + 1, {\bf Abort} if count $\ge c$.
%		\Else
%		\State \textbf{Output} $a_i = \bot$
%		\EndIf
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}



==> estimate_all.tex <==
\mypara{Another strawman method}
 is to let each user report using \olh.
 
After getting reports from users,
the server can estimate the frequency for all possible domains and get the frequent ones.
However, this method is computationally infeasible when the domain size is large.

==> fix_figures.tex <==

%\begin{figure*}[t]
%	\centering
%
%
%    \subfigure[$n = 1000000, m = 64, \epsilon = 4$]{
%		\label{fig:n1000000m64e4_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e4_fix_k}
%	}
%    \subfigure[$n = 1000000, m = 256, \epsilon = 4$]{
%		\label{fig:n1000000m256e4_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m256e4_fix_k}
%	}
%
%    \subfigure[$n = 10000000, m = 64, \epsilon = 4$]{
%		\label{fig:n10000000m64e4_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n10000000m64e4_fix_k}
%	}
%    \subfigure[$n = 10000000, m = 256, \epsilon = 4$]{
%		\label{fig:n10000000m256e4_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n10000000m256e4_fix_k}
%	}
%
%	\caption{Analytical evaluation: FP fixing $k$.}
%	\label{fig:fix_k}
%\end{figure*}

%\begin{figure*}[t]
%	\centering
%	
%	
%	\subfigure[$n = 1000000, m = 64, \epsilon = 4$]{
%		\label{fig:n1000000m64e4_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e4_fix_k}
%	}
%	\subfigure[$n = 1000000, m = 64, \epsilon = 2$]{
%		\label{fig:n1000000m64e2_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e2_fix_k}
%	}
%	
%	\subfigure[$n = 1000000, m = 64, \epsilon = 8$]{
%		\label{fig:n1000000m64e8_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e8_fix_k}
%	}
%	\caption{Analytical evaluation: FP fixing $k$.}
%	\label{fig:fix_k}
%\end{figure*}
%
%\begin{figure*}[t]
%	\centering
%	
%	
%	\subfigure[$n = 1000000, m = 240, \epsilon = 4$]{
%		\label{fig:n1000000m240e4_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_fix_k}
%	}
%	\subfigure[$n = 1000000, m = 240, \epsilon = 2$]{
%		\label{fig:n1000000m240e2_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e2_fix_k}
%	}
%	
%	\subfigure[$n = 1000000, m = 240, \epsilon = 8$]{
%		\label{fig:n1000000m240e8_fix_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e8_fix_k}
%	}
%	\caption{Analytical evaluation: $k$ versus $k / (k + FP)$.}
%	\label{fig:fix_k}
%\end{figure*}

\begin{figure*}[t]
	\centering
	
	
	\subfigure[TP]{
		\label{fig:n1000000m240e4_vary_alpha_TP}
		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_vary_alpha_TP}
	}
	\subfigure[FP]{
		\label{fig:n1000000m240e4_vary_alpha_FP}
		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_vary_alpha_FP}
	}
	
	\subfigure[TP for one segment]{
		\label{fig:n1000000m240e4_vary_alpha_segmentTP}
		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_vary_alpha_segmentTP}
	}
	\subfigure[FP for one segment]{
		\label{fig:n1000000m240e4_vary_alpha_segmentFP}
		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_vary_alpha_segmentFP}
	}
	
	\caption{$n = 1000000, m = 240, \epsilon = 4$ }
	\label{fig:fix_T}
\end{figure*}

\begin{figure*}[t]
	\centering
	
	
	\subfigure[5]{
		\label{fig:n100000m64e2k5p205}
		\includegraphics[width=0.45\columnwidth]{figure/configs/n100000m64e2k5p205}
	}
	\subfigure[6]{
		\label{fig:n100000m64e2k5p206}
		\includegraphics[width=0.45\columnwidth]{figure/configs/n100000m64e2k5p206}
	}
	
	\subfigure[7]{
		\label{fig:n100000m64e2k5p207}
		\includegraphics[width=0.45\columnwidth]{figure/configs/n100000m64e2k5p207}
	}
	\subfigure[8]{
		\label{fig:n100000m64e2k5p208}
		\includegraphics[width=0.45\columnwidth]{figure/configs/n100000m64e2k5p208}
	}
	
	\subfigure[9]{
		\label{fig:n100000m64e2k5p209}
		\includegraphics[width=0.45\columnwidth]{figure/configs/n100000m64e2k5p209}
	}
	\subfigure[10]{
		\label{fig:n100000m64e2k5p2010}
		\includegraphics[width=0.45\columnwidth]{figure/configs/n100000m64e2k5p2010}
	}
	\caption{Fix the candidate size $C=2^5,2^6$,etc, $n = 100000, m = 64, \epsilon = 2$, we vary step length and try to get the the top 32 values. We assume a zipfs distribution for the first 32 values, and zero probability for the rest. All empirical results are averaged on 200 runs.}
	\label{fig:fix_T}
\end{figure*}


\begin{figure*}[t]
	\centering
	
	
	\subfigure[F1 score varying segment size]{
		\label{fig:n1000000m240e4_opt_f1}
		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_opt_f1}
	}
	
	\caption{$n = 1000000, m = 240, \epsilon = 4$ }
	\label{fig:simple_opt}
\end{figure*}


%\begin{figure*}[t]
%	\centering
%
%
%    \subfigure[$n = 1000000, m = 64, \epsilon = 4$]{
%		\label{fig:n1000000m64e4_fix_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e4_fix_T}
%	}
%    \subfigure[$n = 1000000, m = 256, \epsilon = 4$]{
%		\label{fig:n1000000m256e4_fix_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m256e4_fix_T}
%	}
%
%    \subfigure[$n = 10000000, m = 64, \epsilon = 4$]{
%		\label{fig:n10000000m64e4_fix_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n10000000m64e4_fix_T}
%	}
%    \subfigure[$n = 10000000, m = 256, \epsilon = 4$]{
%		\label{fig:n10000000m256e4_fix_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n10000000m256e4_fix_T}
%	}
%
%	\caption{Analytical evaluation: TP / (TP + FP).}
%	\label{fig:fix_T}
%\end{figure*}
%
%\begin{figure*}[t]
%	\centering
%
%
%    \subfigure[$n = 1000000, m = 64, \epsilon = 4$]{
%		\label{fig:n1000000m64e4_vary_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e4_vary_T}
%	}
%\subfigure[$n = 1000000, m = 64, \epsilon = 2$]{
%	\label{fig:n1000000m64e2_vary_T}
%	\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e2_vary_T}
%}
%
%\subfigure[$n = 1000000, m = 64, \epsilon = 8$]{
%	\label{fig:n1000000m64e8_vary_T}
%	\includegraphics[width=0.45\columnwidth]{figure/n1000000m64e8_vary_T}
%}
%    \subfigure[$n = 1000000, m = 256, \epsilon = 4$]{
%		\label{fig:n1000000m256e4_vary_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m256e4_vary_T}
%	}
%
%    \subfigure[$n = 10000000, m = 64, \epsilon = 4$]{
%		\label{fig:n10000000m64e4_vary_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n10000000m64e4_vary_T}
%	}
%    \subfigure[$n = 10000000, m = 256, \epsilon = 4$]{
%		\label{fig:n10000000m256e4_vary_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n10000000m256e4_vary_T}
%	}

%	\caption{Analytical evaluation: TP / (TP + FP).}
%	\label{fig:vary_T}
%\end{figure*}
%
%
%\begin{figure*}[t]
%	\centering
%	
%	\subfigure[$n = 1000000, m = 240, \epsilon = 2$]{
%		\label{fig:n1000000m240e2_vary_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e2_vary_T}
%	}
%	\subfigure[$n = 1000000, m = 240, \epsilon = 4$]{
%		\label{fig:n1000000m240e4_vary_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_vary_T}
%	}
%	
%	
%	\subfigure[$n = 1000000, m = 240, \epsilon = 8$]{
%		\label{fig:n1000000m240e8_vary_T}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e8_vary_T}
%	}
%	\caption{Analytical evaluation: $\EV{TP} / (\EV{TP} + FP)$.}
%	\label{fig:vary_T}
%\end{figure*}
%
%\begin{figure*}[t]
%	\centering
%	
%	\subfigure[$n = 1000000, m = 240, \epsilon = 2$]{
%		\label{fig:n1000000m240e2_vary_T_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e2_vary_T_f}
%	}
%	\subfigure[$n = 1000000, m = 240, \epsilon = 4$]{
%		\label{fig:n1000000m240e4_vary_T_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e4_vary_T_f}
%	}
%	
%	
%	\subfigure[$n = 1000000, m = 240, \epsilon = 8$]{
%		\label{fig:n1000000m240e8_vary_T_k}
%		\includegraphics[width=0.45\columnwidth]{figure/n1000000m240e8_vary_T_f}
%	}
%	\caption{Analytical evaluation: F1 score.}
%	\label{fig:vary_T_k}
%\end{figure*}

==> general_prot.tex <==
%\subsection{A General Protocol}
In the high level, protocols following \covt work as follows:
First, the aggregator specifies some parameters to each user. 
Then each user reports based on his private input and the parameter.
Finally the server aggregates and analyzes the results from all users and finds out the heavy hitters.

The users are partitioned into groups, and users in the same group will receive the same parameter.
\olh, described in Section~\ref{subsubsec:olh}, is used to report the substring of the private value. Assume the values are represented by strings. 

Algorithm~\ref{alg:covt_server} and~\ref{alg:covt_user} presents the server/local part of the protocol:

\begin{algorithm}
	\caption{Aggregator}\label{alg:covt_server}
	\begin{algorithmic}[1]
		\Require \covt
		\Ensure $k$ values.
		\Procedure{Find}{\covt}
		\State $nn\leftarrow$ number of non-leaf nodes in \covt.
		\For{each non-leaf node $u\in\covt$}
			\State Sample $n/nn$ users without replacement.
			\State Send $L(u)$ to these users.
		\EndFor
		\State Assign $\{0,1\}$ to each leaf node.
		\State Topologically sort non-leaf nodes and get $V$.
		\For{$u\in V$}
			\State Construct candidate set.
			\State Receive reports $\{r\}$ from users on $u$.
			\State Feed $\{r\}$ to the frequency oracle.
			\State Query the oracle about each candidate.
			\State 
		\EndFor
		\State \textbf{return} sorted $\{R^i\}$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

Note that the topology sort guarantees the algorithm always proceed with non-leaf nodes without dependency, 
or with nodes whose dependencies are all ready.

\begin{algorithm}
	\caption{Local Randomizer}\label{alg:covt_user}
	\begin{algorithmic}[1]
		\Require Private value $v$, a label $L(u)$.
		\Ensure Report $r$.
		\Procedure{Rand}{$v, L(u)$}
		\State Get $st\leftarrow min\{L(u)\}, ed\leftarrow max\{L(u)\}$.
		\State Truncate $v$ into substring $v'\leftarrow v[st,ed]$.
		\State Encode $v'$ into $v''\leftarrow \mathsf{Encode}(v')$
		\State Perturb $v''$ into $r\leftarrow \mathsf{Perturb}( v'')$.
		\State \textbf{return} $r$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\begin{comment}
\begin{itemize}
	\item From the user side:
	\begin{itemize}
		\item 
		\mypara{Encoding.}
		The aggregator specifies the start and end positions, $st, ed$, of the report.
		The user first truncates the value $v$ to get $v[st,ed]$, the substring from $st$ to $ed$.
		$v[st,ed]$ is then encoded: $v'=\mathsf{Encode}(v[st,ed])$.
		\item 
		\mypara{Perturbation.}
		The perturbation algorithm from \OLH is used:
		$\mathsf{Perturb}( v')= r$. 
	\end{itemize}
	\item From the server side:
	\begin{itemize}
		\item
		\mypara{Identification.}
		$\mathsf{Aggregate}$ from the LDP primitive is used to estimate frequencies of patterns in a dictionary. Those with estimated frequencies above a threshold are identified as candidates. The dictionary is the set of all possible combinations of partial candidates, or just all possibilities if the current segment is the most fine-grained.
	\end{itemize}
\end{itemize}
\end{comment}

==> hash2.tex <==
\subsection{\simhash}
\label{subsec:hash}
The high-level intuition of using hash functions is to separate values into different channels, such that the probability different heavy hitters are transmitted via the same channel is small. Users report with noise satisfying LDP in the channel where his value is hashed into, and pure noise in all other channels. Therefore, in each channel, at most one (could be multiple, described below) candidate will be detected for each segment. The concatenation of all segment candidates is the resulted candidate in the current channel.

Based on the observations made from \hash protocol, we propose a simpler protocol as follows:
Instead of reporting one bit, each user reports a segment of $s$ bits. Instead of using \blh, the optimized \olh (or \oue, when the computation is tolerable) can be used. No error correction code will be used.

\mypara{Error Handling.}
In order to handle errors during estimation, \hash uses error correction code and list decoding. However, in the case of \simhash, since there are fewer groups ($m/s$ instead of $m$ groups), the estimation will be more accurate, and thus, less errors will happen. (Note that in \hash, an error means the detected value is wrong, while in \simhash, an error means none of the estimated frequency passes the significance threshold.) In this case, when an error happens, we can enumerate all possibilities in that position, and when too many errors happen (e.g., more than one), we take that as non-candidate and discard the result in this channel.

\mypara{Collision Handling.}
We observe that, when multiple heavy hitters are hashed into the same channel, we can detect all the collided values in a single channel: We can detect all of them for all segments, and they came up with similar order. Therefore, we propose to take the candidates in each segment that come out first and concatenate them as a candidate, all that come out second, etc.

Formally, the protocol runs as follows:

\mypara{Encoding.}
$\mathsf{Encode}(v)=\langle P, \mathbf{B_0}\rangle$ where $p\in[m/s]$ is a location in the value, and $\mathbf{B_0}$ is a $t$ long
vector such that $\mathbf{B_0}[H(v)]=v$ and $\mathbf{B_0}[i]=\bot$ for $i \neq H(v)$. $H(\cdot)$ is the pre-agreed hash function from $[d]$ to $[t]$. $t$ is a value dependent on $\sqrt{n}$.

\mypara{Perturbation.}
$\mathsf{Perturb}(\langle p, \mathbf{B_0}\rangle)=\langle p, \mathbf{B}\rangle$, where $\mathbf{B}$ is a $t$ long
vector, and $\forall i \in [t]$, if $i=H(v)$, $B[i]=\mathsf{Perturb_{prim}}(\mathbf{B_0}[i][p\cdot s:(p+1)\cdot s])$; otherwise, $B[i]\xleftarrow{\$}\{0,1\}^s$.

\mypara{Identification.}
For each channel $i$, a candidate or $\bot$ will be generated: Given reports $\{\langle p,\mathbf{B}[k] \rangle\}$, first find candidates for every segment $p\in[m/s]$, and then concatenate them to get a candidate. 

Note that because of the pure noise added by all users not belonging to the current channel, we need to subtract an amount of pure noise, $n/t$, to get the real estimate. There's no iterations in this protocol.




==> maxent.tex <==
\subsection{MAX-ENT}
%The intuition is to divide the big domain size into smaller pieces,
%and then analyze them together.
%Hopefully,
%during the process of reconstructing joint distributions,
%we are able to filter some candidates we are not interested.
%Thus, we are able to get the information we want.
%
%For example, we want to estimate the frequency of hashes of passwords,
%the domain size is $2^{128}$, which is prohibitive to compute.
%But it is much easier to compute using $16$ channels, 
%$Ch^1, Ch^2, \ldots, Ch^{16}$,
%each transmitting $8$ bits 
%(with privacy budget divided by $16$,
%and the choice of frequency oracle depends on the estimated variance).
%We use $D^i$ to denote the domain of the $i$-th channel
%(in this case, $D^i = [2^8]$),
%and $R^i(v) \subset [d]$ to denote the set candidates (from $[d]$) that is projected into $v$ (from $D^i$) in the $i$-th channel
%(in this case, $R^i(v) = \{x|x\in[d]\wedge i\mbox{-th 8-bit segment of }x=v\})$. 
Different from \mle, \maxent only requires estimation in each channel. 
Thus, it is possible to partition the population into groups, and each user only answer one question (instead of multiple questions).

\mypara{Encoding.}
$\mathsf{Encode}(v)=\langle p, x\rangle$ where $p\in[m]$, and $x=\mathsf{Encode}_{prim}(G^{p}(v))$.

\mypara{Perturbation.}
$\mathsf{Perturb}(\langle p, x\rangle)=\langle p, y\rangle$, where $y=\mathsf{Perturb}_{prim}(x)$.

\mypara{Identification.}

{\it (Step 1) Marginal Estimate.}
Given reports $\langle p^j, y^j\rangle$'s, the aggregated estimate for each channel is generated:
\begin{align*}
\tilde{c}^p=\mathsf{Aggregate}(\{y^j | j\in [n], p^j=p\})
\end{align*}

{\it (Step 2) Max-Ent Estimation.}
Apply the principle of Maximum Entropy to get an estimation of the whole distribution.

\mypara{Cost.} Estimating frequency in each channel is efficient. The runtime of the optimization algorithm depends on the termination condition.

\mypara{Privacy.}
This LDP primitive satisfies is $\epsilon$-LDP.

\mypara{Max-Ent}


%During the combining phase,
%we need to filter out some infrequent candidates,
%so that it is feasible to analyze the distribution of frequent full strings.
%The filtering threshold is a tradeoff between accuracy and time complexity.
%False negatives may happen if the threshold is high.

%Initial filtering may lead to missing of frequent full strings 
%(e.g., $\Pr{8\mbox{ zeros}} = \frac{1}{2^8}$ in $Ch^1$,
%but they all comes from the same full-string candidate, i.e.,
%$\Pr{128\mbox{ zeros}} = \frac{1}{2^8}$ in the full string).

%After getting partial distributions of each category,
%we need to find the joint distribution.
%For example,
%we have $\Pr{A_1} = 0.6, \Pr{A_2} = 0.4$,
%and $\Pr{B_1} = 0.5, \Pr{B_2} = 0.5$,
%we want to estimate 
%$\Pr{A_1,B_1}, \Pr{A_1,B_2}, \Pr{A_2,B_1}, \Pr{A_2,B_2}$.

%A common approach to use in the combining phase is to apply the Principle of Maximum Entropy.
Intuitively speaking,
with constraints fixed,
the distribution with maximal entropy is always close to
the real distribution.

%Suppose we are estimating distribution over $c$ channels, $Ch^1, Ch^2, \ldots, Ch^c$.
%We denote $\tilde{c}_{v_1,v_2,\ldots, v_c}$ as the summation of estimated frequency of candidates 
%in the whose value in the $i$-th channel is $v_i$, 
%or
%$\tilde{c}_{v_1,v_2,\ldots, v_c} = \sum_{i\in\bigwedge_{ch\in[c]} R(Ch^{ch}, v_{ch})}\tilde{c}_j$.
%For simplicity, we use shortcuts such as $\tilde{c}_{v_i}$ for $\tilde{c}_{v_1,v_2\ldots,v_c}$ when the context is clear.
%Formally, Principle of Maximum Entropy is an optimization problem:
%\begin{align*}
%%\mbox{maximize}&-\frac{\tilde{c}(i)}{n}\log\frac{\tilde{c}(i)}{n}\\
%\mbox{maximize }&-\tilde{c}_{v_i}\log\tilde{c}_{v_i}\\
%\mbox{subject to }&\forall ch\in[c], d\in D(Ch^{ch}):\\
%&\sum_{i\in[c]\setminus ch, v_i\in D(Ch^i)} \tilde{c}_{v_1,v_2,\ldots,v_{ch-1},d,v_{ch+1},\ldots,v_c} = \tilde{c}^{ch}_d,
%\end{align*}
%where $\tilde{c}^{ch}_d$ results from the random oracle used in the previous phase.
%This process should be applied gradually
%(e.g., combining two channels at a time, recursively bottom up)
%to be efficient 
%(combining all channels at once leads to $2^{128}$ candidates,
%which is obviously infeasible).

Note that the optimization phase can be applied to all the channels at once or several (e.g., two) channels iteratively.

%Figure~\ref{fig:2-bit} and~\ref{fig:all-bit} shows result of analyzing frequency of six-bit strings.
%We use three channels each transmitting two bits.
%After getting the estimation of every two-bit substrings (as shown in Figure~\ref{fig:2-bit}),
%we estimate the joint distribution by applying the Principle of Maximum Entropy.
%An off-the-shelf optimization tool, CVXOPT~\cite{cvxopt} is used in our experiment.
%For simplicity, 
%we do not filter any candidate strings.
%\begin{figure*}[t]
%	\centering
%	\subfigure[{$C_i \mbox{ and } \tilde{c}(i)$ of first two bits}]{
%		\label{fig:12bit}
%		\includegraphics[width=0.63\columnwidth]{figure/count-3}
%	}	
%	\subfigure[{$C_i \mbox{ and } \tilde{c}(i)$ of middle two bits}]{
%		\label{fig:34bit}
%		\includegraphics[width=0.63\columnwidth]{figure/count-2}
%	}
%	\subfigure[{$C_i \mbox{ and } \tilde{c}(i)$ of last two bits}]{
%		\label{fig:56bit}
%		\includegraphics[width=0.63\columnwidth]{figure/count-1}
%	}
%	\caption{
%		Each subfigure shows frequency of two-bit strings.	
%		We use $\epsilon=1$, $d=2^6$, $n = 10000$ samples, 
%		and assume the strings are sampled in Zipf's distribution. 
%		We use \protRandom{} to estimate counts.
%		Each two-bit string consumes a privacy budget of $\epsilon/3$.}
%	\label{fig:2-bit}
%\end{figure*}
%
%\begin{figure*}[t]
%	\centering
%	\subfigure[Synthesized {$C_i \mbox{ and } \tilde{c}(i)$ of all possible strings}]{
%		\label{fig:allbit}
%		\includegraphics[width=1.95\columnwidth]{figure/count-0}
%	}	
%	\caption{
%		Estimated frequency of six-bit strings.
%		Result is synthesized by the Max-Entropy principle.
%		For simplicity,
%		We do not filter any candidates.
%		Statistics of two-bit strings got in Figure~\ref{fig:2-bit}.
%	}
%	\label{fig:all-bit}
%\end{figure*}

==> norm_inv.tex <==

\begin{table*}[t]
	\centering
	\hspace*{-1pt}\makebox[\linewidth][c]{\begin{tabular}{| c | c |}
			\hline
			 $m$ & $Q$\\ \hline

$16$&$4.81$\\ \hline
$24$&$5.82$\\ \hline
$32$&$6.68$\\ \hline
$48$&$8.13$\\ \hline

	\end{tabular}}
	\caption{Q value.}
	\label{table:norm_inv}
\end{table*}



==> prod.tex <==
%\subsection{\itergroup and \product}
\begin{comment}
% shortened discription when we have the covertree structure
The \covt guides the aggregator about which bits to analyze.
For each $m$, there exists multiple \covt.
We highlight two protocols derived from two special cases of \covt in Figure~\ref{fig:protocols_trees},
\itergroup and \product.
In the \covt for \itergroup,
each node $u[i]$ takes candidate sets from exactly one node child $u[i-1]$ and $s[i]$ leaves.
The first node $u[1]$ is special. It does not have node child.
In \itergroup,
the aggregator first takes a segment of $s[1]$ bits, finds out frequent patterns as $C(u[1])$,
and then extends the segment to $s[1]+s[2]$ bits.
Note that now the aggregator does not need to check for all the possible values,
instead, he only needs to check for values whose first $s[1]$ bits are identified as frequent.
The intuition is that,
if a value is frequent, any part of it must also be frequent.
The aggregator repeats this operation until the he finds out the candidate set for the root node,
which is essentially the frequent patterns in the full domain.

Different from \itergroup, which expands the segment linearly,
\product works in a bottom-up manner.
The \covt for it is very balanced. 
This enables parallel processing on nodes in the same layer.

We use \itergroup in the actual analysis and implementation, 
since the linear structure of \itergroup makes it easier to analyze.
\end{comment}


\begin{comment}
% the following formal description and example may not be necessary anymore once the \covt algorithm is given
In the high level, the identification stage of \product works in a bottom-up manner: For each of the non-overlapping segments of the string, the aggregator queries the frequency estimator on all possible patterns and finds out frequent patterns.
Then some of those segments are grouped together and frequent patterns in this larger segments are identified.
To find frequent patterns in a larger segment, testing every pattern may be inefficient and error-prone.
Thus, the aggregator only tests patterns whose parts are already identified as frequent.
The intuition is that, a frequent string must be composed of substrings that are also frequent.
The resulting frequent patterns can then be used for even larger segments in the next phase.
This process can be repeated multiple times until the full-string heavy hitters are identified. 
%In practice, we group two or three segments together. 
%If a substring cannot be grouped with others, this merging operation for it will be delayed unless in the final phase.
%Users are partitioned evenly into groups. Different groups report different parts of their values as indicated by the aggregator.





An example of the process of identifying heavy hitters for 5-character strings is illustrated in Figure~\ref{fig:hie_diag}. 
Users are partitioned evenly into seven groups.
Five groups of users report based on one of the five characters,
one group of users report based on the first three characters,
and one report the full string.
After getting the reports from users,
the aggregator first analyzes reports on each character.
For each set of reports, the aggregator queries all possible characters and identifies two most frequent ones.
Then the aggregator analyzes reports on the first three characters, and finds two most frequent three-character patterns. The aggregator only tests eight values, since the frequent 3-character patterns are highly likely to be composed of frequent letters in each position, and the frequent characters in each location are already know.
The fourth and fifth characters are delayed until final analysis, 
where the first three characters, the fourth character, and the fifth character are analyzed together to find the full-string heavy hitters.
\end{comment}
%In this case, letter `h', `w' are frequent in the first position, `e', `o' are frequent in the second, and `l', `r' are frequent in the third. Therefore, the candidate set of patterns to be tested is $\{\mbox{`hel', `}\}

%Suppose each user's value $v\in\{0,1\}^m$, and the most fine-grained segment length $s$. There are $\log (m/s)$ layers in the tree, and each node will receive a domain $D$, and output a set of candidates $C\subset D$. 

%The internal process of each node works as follows: every user in each leaf node group will receive $D=\{0,1\}^s$ and run an LDP primitive, encode and report a length-$s$ substring (same part for all users in a group, e.g., every user encodes his fourth bit to eighth bit, but different groups encode different, none-overlapping parts), with an aggregator, who will aggregate the reports, find the candidates with the estimated frequency above a pre-determined threshold, and output these candidates. The domain for the users in a non-leaf node $G^{i,j}$ is the set of every possible concatenation of the two candidates (Cartesian product) from the two children nodes. For example, in Figure~\ref{fig:hie_diag}, $C^{1,0}=\{de,be\}, C^{1,1}=\{ad,ef\}$, $D^{0,0}=\{dead,deef,bead,beef, \bot\}$. $\bot$ is a special ``none'' category (for users to indicate his value does not fall into any of the combinations), which is used for any non-leaf node. This process continues until the root node outputs the candidate set, which is the final result.

%Specifically, $G^{i,j}$ (the $j$-th node in level $i$) will receive frequent items (candidate) from its two children, that is, candidates for two substrings of length $m/2^{i+1}$, and output candidates for the $j$-th $m/2^i$-bit long substring. Leaf nodes will receive nothing. For example, the input to the root node is the output of its two children, the frequent segments for the first half and second half, respectively. 



 
%In this protocol, a tree-based structure is used. Each node receives a list of values as domain, and outputs a list of values as candidates. Similar amount of users are assigned to every node of the tree. What a user reports depends on the which node he is assigned. Suppose the user's value is a fixed length string. Users in the leaf nodes report the most fine-grained consecutive and non-overlapping segments, and users in each non-leaf node report the concatenation of segments from the children nodes. The domains in the leaf nodes are all the possibilities of the segment, and the domain of each non-leaf node is the concatenation of every combination of candidates in its children nodes, besides a special ``none'' category.
%
%For instance, suppose the value is a fixed-length string of $8$ bytes, and assume a three-layer binary tree is used. Users in the four leaf nodes report segment of two bytes, and users in the second layer reports four bytes concatenating of the two segments in the children nodes, only if both segments are identified as candidates; otherwise the users report the special category of ``none''. For users in the root node, the full strings are reported, only if both four-byte segment are identified as candidates in the two second layer nodes.
%
%Define $L_i$ as the $i$-th layer of the tree. $L_0$ is the bottom layer, which contains $m/s$ nodes, $L_0=\{node_{0,1}, node_{0,2},\ldots, node_{0,m/s}\}$ (each node $node_{i, j}$ corresponds to the $j$-th $2^im/s$-long segment), $L_{\log (m/s)}$ is the top layer, which contains the root node, $L_{\log (m/s)}=\{node_{{\log (m/s)}, 1}\}$.
%Define $N$ as the union of all nodes, i.e., $N=\bigcup_{i=0}^{\log(m/s)}L_i$.

%Each node $node_{i, j}$ takes a candidate list $C\subseteq\{0,1\}^{2^im/s}$ and outputs $C'\subseteq\{0,1\}^{2^im/s}$. We override two operations: 
%\begin{itemize}
%	\item We say a value $v\in C$ in $node_{i,j}$ if the $j$-th $2^im/s$-long segment of $v$, i.e., $v[(j-1)2^im/s:j2^im/s]\in C$. 
%	\item We define the Cartesian product of two candidate lists output by $node_{i,j}$ and $node_{i,j+1}$ (assuming $j$ is odd) as follows: $C_{i, j}\times C_{i,j+1}=\{c=c||c': c\in C_{i,j}\wedge c'\in C_{i,j+1}\}$.
%\end{itemize}

\begin{comment}
Formally, \product works as follows:

\begin{itemize}
	\item From the user side:
	\begin{itemize}
		\item 
			\mypara{Encoding.}
			The aggregator specifies the start and end positions, $st, ed$, of the report.
			The user first truncates the value $v$ to get $v[st,ed]$, the substring from $st$ to $ed$.
			$v[st,ed]$ is then encoded: $v'=\mathsf{Encode}(v[st,ed])$.
		\item 
			\mypara{Perturbation.}
			The perturbation algorithm from \OLH is used:
			$\mathsf{Perturb}( v')= r$. 
	\end{itemize}
	\item From the server side:
	\begin{itemize}
		\item
			\mypara{Identification.}
			$\mathsf{Aggregate}$ from the LDP primitive is used to estimate frequencies of patterns in a dictionary. Those with estimated frequencies above a threshold are identified as candidates. The dictionary is the set of all possible combinations of partial candidates, or just all possibilities if the current segment is the most fine-grained.
	\end{itemize}
\end{itemize}

\end{comment}

\begin{comment}
\begin{figure}[t]
	\centering
	\subfigure[\product]{
		\label{fig:hie_diag}
		\includegraphics[width=0.5\columnwidth]{figure/prod}
	}
	\subfigure[\itergroup]{
		\label{fig:iter_diag}
		\includegraphics[width=0.4\columnwidth]{figure/iter}
	}
	\caption{Illustrative examples of protocols \product and \itergroup. Each cylinder represents a database, containing reports on a specific substring, denoted by the black part of the rectangle. The dashed rectangle is the aggregation process from the aggregator, and the frequent pattern are identified in the brackets.}
	\label{fig:protocols_comp}
\end{figure}
\end{comment}

==> product.tex <==



==> sort.tex <==
\mypara{A strawman method}
 is to let each user report a perturbed value.
This requires using Protocol \protRandom{} as the frequency oracle,
which is not good when the domain size is big (the current setting). 

After getting reports from users in the format of a random response,
the server can sort them (either in the form of quick sort or tree-based sort),
and then rescale them. 
Since there are $n$ reports,
there are at most $n$ items after sorting,
and after rescaling,
the unfiltered candidates (appears some times after rescaling) should be less.
